Towards Unifying Medical Vision-and-Language Pre-training via Soft Prompts

Medical vision-and-language pre-training (Med-VLP) has shown promising improvements on many downstream medical tasks owing to its applicability to extracting generic representations from medical images and texts. Practically, there exist two typical types, \textit{i.e.}, the fusion-encoder type and the dual-encoder type, depending on whether a heavy fusion module is used. The former is superior at multi-modal tasks owing to the sufficient interaction between modalities; the latter is good at uni-modal and cross-modal tasks due to the single-modality encoding ability. To take advantage of these two types, we propose an effective yet straightforward scheme named PTUnifier to unify the two types. We first unify the input format by introducing visual and textual prompts, which serve as a feature bank that stores the most representative images/texts. By doing so, a single model could serve as a \textit{foundation model} that processes various tasks adopting different input formats (\textit{i.e.}, image-only, text-only, and image-text-pair). Furthermore, we construct a prompt pool (instead of static ones) to improve diversity and scalability. Experimental results show that our approach achieves state-of-the-art results on a broad range of tasks, spanning uni-modal tasks (\textit{i.e.}, image/text classification and text summarization), cross-modal tasks (\textit{i.e.}, image-to-text generation and image-text/text-image retrieval), and multi-modal tasks (\textit{i.e.}, visual question answering), demonstrating the effectiveness of our approach. Note that the adoption of prompts is orthogonal to most existing Med-VLP approaches and could be a beneficial and complementary extension to these approaches.

==> tables/dataset.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1mm}{\begin{tabular}{@{}l|rrcc@{}}
\toprule
Datasets  & Image \# & Text \#  & Avg. Len. & Avg. Sent. \#  \\ \midrule
ROCO      &  81k     &  81k     & 20.42     &  1.46          \\
MedICaT   & 124k     & 321k     & 40.88     &  2.82          \\
MIMIC-CXR & 232k     & 367k     & 36.49     &  5.07          \\ \bottomrule
\end{tabular}}
\caption{The statistics of the three pre-training datasets including the numbers of images, texts, the average word-based length (Avg. Len.) of texts, and the average number of sentences (Avg. Sent. \#).}
\label{table:datasets}
\end{table}
